InvariantOODG: Learning Invariant Features of Point Clouds for Out-of-Distribution Generalization

The convenience of 3D sensors has led to an increase in the use of 3D point clouds in various applications. However, the differences in acquisition devices or scenarios lead to divergence in the data distribution of point clouds, which requires good generalization of point cloud representation learning methods. While most previous methods rely on domain adaptation, which involves fine-tuning pre-trained models on target domain data, this may not always be feasible in real-world scenarios where target domain data may be unavailable. To address this issue, we propose InvariantOODG, which learns invariability between point clouds with different distributions using a two-branch network to extract local-to-global features from original and augmented point clouds. Specifically, to enhance local feature learning of point clouds, we define a set of learnable anchor points that locate the most useful local regions and two types of transformations to augment the input point clouds. The experimental results demonstrate the effectiveness of the proposed model on 3D domain generalization benchmarks.

==> samples/02_related_works.tex <==
\vspace{-0.1in} 
\subsection{3D Point Cloud Learning}
Significant progress has been made in point cloud classification and detection using simulated and real-world data \cite{qi2017pointnet,qi2017pointnet++,wang2019dgcnn}.
PointNet\cite{qi2017pointnet}  and PointNet++\cite{qi2017pointnet++} are popular deep neural network architectures, but PointNet has limitations in recognizing fine-grained patterns and complex scenes. PointNet++ addresses this by capturing local features hierarchically.
Other methods, such as PointCNN \cite{li2018pointcnn}, PCNN \cite{atzmon2018point}, and Graph Convolutional Neural Networks, have also contributed to the field of point cloud feature learning.
However, these methods assume training and test data belong to the same domain and have similar distributions, which is often inconsistent in practice.


\vspace{-0.1in} 

\subsection{Domain Adaptation}

Domain adaptation is a crucial technique in machine learning that enables models to transfer from a source domain with abundant labeled data to a target domain with scarce or non-existent labeled data.
This is especially important when there is a significant difference between the training and testing data.
Unsupervised domain adaptation (UDA) is a challenging task that relies solely on unlabeled target domain data.

Extensive research has been conducted on UDA methods tailored to image data, including adversarial training \cite{ganin2015unsupervised, ganin2016domain, purushotham2017variational} and minimizing divergence between source and target domains\cite{long2015learning, sun2016deep, zhang2018aligning}. 



 In recent years, there has been a growing interest in UDA research for 3D point clouds. While some studies \cite{saleh2019domain, wu2019squeezesegv2}  have adapted 2D image domain adaptation techniques to process 3D point clouds, this approach results in a significant loss of crucial 3D geometric information. Several UDA methods specifically designed for point cloud data have been proposed, including adapting local and global features and harnessing generative models for domain adaptation \cite{qin2019pointdan, sauder2019self,achituve2021self}. 
 However, these methods assume the availability of target domain data, which can be challenging or expensive in real-world scenarios.




\vspace{-0.1in} 
\subsection{Out-of-Distribution Generalization}

The problem of Out-of-Distribution generalization (OODG) addresses a challenging scenario where the distribution of the testing data is unknown and differs from the training data's distribution \cite{shen2021towards}.

 Various techniques have been developed to address this problem, including causation \cite{yang2021causalvae, shen2022weakly}, representation learning \cite{bengio2013representation, locatello2019challenging} and optimization-based approaches\cite{chang2020invariant}. 
 However, limited attention has been given to OODG for point clouds. Only a few studies have explored this problem. Metasets \cite{huang2021metasets} introduces four data augmentation modes applied to CAD datasets to simulate possible defects in real-world point cloud data. Wei \textit{et al.} \cite{wei2022learning} constructed a shared partial template feature spatial domain between the source and target domains based on learning domain-independent features.
 In this paper, we propose a novel approach that focuses on local-to-global learning using anchor points to optimize invariance learning of local and global features. Our method addresses the limitations of existing methods and provides experimental evaluations to demonstrate its effectiveness and robustness.



